Modelling of Underwater Vehicles using Physics-Informed Neural Networks with Control

Physics-informed neural networks (PINNs) integrate physical laws with data-driven models to improve generalization and sample efficiency. This work introduces an open-source implementation of the Physics-Informed Neural Network with Control (PINC) framework, designed to model the dynamics of an underwater vehicle. Using initial states, control actions, and time inputs, PINC extends PINNs to enable physically consistent transitions beyond the training domain. Various PINC configurations are tested, including differing loss functions, gradient-weighting schemes, and hyperparameters. Validation on a simulated underwater vehicle demonstrates more accurate long-horizon predictions compared to a non-physics-informed baseline

==> tables/activation_function_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!b]
\centering
\caption{Comparison of adaptive activation functions on performance metrics.}
\label{tab:activation_function}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|}
\textbf{Adaptive Activation Function}       & \textbf{Softplus} & \textbf{tanh} \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $-4.85$           & $\bm{-5.13}$  \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $-3.37$           & $\bm{-3.64}$  \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-2.67}$      & $-2.57$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.99$           & $\bm{-5.35}$  \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.70$           & $\bm{-4.89}$  \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $\bm{1.51}$/$18.9$ & $0.96$/$12.0$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $\bm{1.27}$/$21.2$ & $1.17$/$19.5$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{1.46}$/$14.6$ & $0.86$/$8.60$
\end{tabular}
%}

\end{table}

==> tables/architecture_subtables.tex <==
% \begin{table}[!b]
% \centering
% \caption{Overview of architecture experimental results}
% \label{tab:architecture_experiments}
% \begin{subtable}{\columnwidth}
%     \caption{Neural network size experiment}
%     \label{tab:nn_size_exp}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r|r|r|r}
%     \textbf{NN Size $N_{layer}$/$N_h$}             & \textbf{4/32} & \textbf{3/32} & \textbf{5/32} & \textbf{4/16} & \textbf{4/64} \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$            & $-4.85$       & $-4.78$       & $-4.51$       & $\bm{-5.04}$  & $-4.93$       \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$            & $-3.37$       & $-3.27$       & $-2.94$       & $\bm{-3.56}$  & $-3.47$       \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$             & $-2.67$       & $-2.25$       & $-2.56$       & $\bm{-2.69}$  & $-2.60$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$    & $-4.99$       & $-4.90$       & $-4.69$       & $\bm{-5.24}$  & $-5.16$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$    & $-4.70$       & $-4.60$       & $-4.37$       & $\bm{-4.87}$  & $-4.74$       \\ \hline
%     $\text{VPT}_{dev}$ {[}s{]}/{[}steps{]}         & $\bm{1.51}$/$18.9$ & $1.23$/$15.4$ & $0.58$/$7.25$ & $1.36$/$17.0$ & $1.12$/$14$   \\ \hline
%     $\text{VPT}_{test,interp}$ {[}s{]}/{[}steps{]} & $1.27$/$21.2$ & $0.62$/$10.3$ & $0.46$/$7.67$ & $\bm{1.32}$/$22.0$ & $1.16$/$19.3$ \\ \hline
%     $\text{VPT}_{test,extrap}$ {[}s{]}/{[}steps{]} & $\bm{1.46}$/$14.6$ & $1.31$/$13.1$ & $0.58$/$5.8$  & $1.31$/$13.1$ & $1.11$/$11.1$
%     \end{tabular}%
%     }
% \end{subtable}

% \vspace{1em} 

% \begin{subtable}{\columnwidth}
%     \caption{Residual connection ablation experiment}
%     \label{tab:ress_conn}
%     \centering
%     %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r}
%     \textbf{Residual Connection}                   & \textbf{With} & \textbf{Without} \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$            & $\bm{-4.85}$  & $-0.69$          \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$            & $\bm{-3.37}$  & $2.09$           \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$             & $\bm{-2.67}$  & $-0.83$          \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$    & $\bm{-4.99}$  & $-0.79$          \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$    & $\bm{-4.70}$  & $-0.61$          \\ \hline
%     $\text{VPT}_{dev}$ {[}s{]}/{[}steps{]}         & $\bm{1.51}$/$18.9$ & $0.00$/$0.00$    \\ \hline
%     $\text{VPT}_{test,interp}$ {[}s{]}/{[}steps{]} & $\bm{1.27}$/$21.2$ & $0.00$/$0.00$    \\ \hline
%     $\text{VPT}_{test,extrap}$ {[}s{]}/{[}steps{]} & $\bm{1.46}$/$14.6$ & $0.00$/$0.00$   
%     \end{tabular}
%     %}
% \end{subtable}

% \vspace{1em} 

% \begin{subtable}{\columnwidth}
%     \centering
%     \caption{Adaptive activation function comparison}
%     \label{tab:activation_function}
%     %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r}
%     \textbf{Adaptive Activation Function}       & \textbf{\lstinline|softplus|} & \textbf{\lstinline|tanh|} \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$         & $-4.85$           & $\bm{-5.13}$  \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$         & $-3.37$           & $\bm{-3.64}$  \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-2.67}$      & $-2.57$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.99$           & $\bm{-5.35}$  \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.70$           & $\bm{-4.89}$  \\ \hline
%     $\text{VPT}_{dev}$ [s]/[steps]              & $\bm{1.51}$/$18.9$ & $0.96$/$12.0$ \\ \hline
%     $\text{VPT}_{test,interp}$ [s]/[steps]      & $\bm{1.27}$/$21.2$ & $1.17$/$19.5$ \\ \hline
%     $\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{1.46}$/$14.6$ & $0.86$/$8.60$
%     \end{tabular}
%     %}
% \end{subtable}
% \end{table}





==> tables/batch_size_no_pinn_table.tex <==
\begin{table}[!b]
\centering
\caption{Batch size experiment without physics and rollout loss.}
\label{tab:batch_size_no_pinn}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|r|}
\textbf{Batch Size}                         & \textbf{3}    & \textbf{10}   & \textbf{30}   \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $-4.45$       & $\bm{-4.76}$  & $-4.56$       \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $-2.89$       & $\bm{-3.38}$  & $-3.03$       \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-1.84}$  & $-1.81$       & $-1.83$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.81$       & $\bm{-4.87}$  & $-4.79$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.16$       & $\bm{-4.47}$  & $-4.30$       \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $0.46$/$5.75$ & $\bm{1.49}$/$18.6$ & $0.82$/$10.3$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $0.42$/$7.00$ & $1.23$/$20.5$ & $\bm{1.35}$/$22.5$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $0.48$/$4.70$ & $\bm{0.85}$/$8.50$ & $0.64$/$6.40$
\end{tabular}
%}
\end{table}

==> tables/batch_size_subtables.tex <==
% \begin{table}[!b]
% \centering
% \caption{Batch size experiments}
% \label{tab:batch_size_experiments}
% \begin{subtable}{\columnwidth}
%     \centering
%     \caption{Without physics and rollout loss}
%     \label{tab:batch_size_no_pinn}
%     %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r|r}
%     \textbf{Batch Size}                         & \textbf{3}    & \textbf{10}   & \textbf{30}   \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$         & $-4.45$       & $\bm{-4.76}$  & $-4.56$       \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$         & $-2.89$       & $\bm{-3.38}$  & $-3.03$       \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-1.84}$  & $-1.81$       & $-1.83$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.81$       & $\bm{-4.87}$  & $-4.79$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.16$       & $\bm{-4.47}$  & $-4.30$       \\ \hline
%     $\text{VPT}_{dev}$ [s]/[steps]              & $0.46$/$5.75$ & $\bm{1.49}$/$18.6$ & $0.82$/$10.3$ \\ \hline
%     $\text{VPT}_{test,interp}$ [s]/[steps]      & $0.42$/$7.00$ & $1.23$/$20.5$ & $\bm{1.35}$/$22.5$ \\ \hline
%     $\text{VPT}_{test,extrap}$ [s]/[steps]      & $0.48$/$4.70$ & $\bm{0.85}$/$8.50$ & $0.64$/$6.40$
%     \end{tabular}
%     %}
% \end{subtable}

% \vspace{1em}

% \begin{subtable}{\columnwidth}
%     \centering
%     \caption{With physics and rollout loss}
%     \label{tab:batch_size_with_pinn}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r|r|r|r}
%     \textbf{Batch Size}                         & \textbf{3}    & \textbf{10}   & \textbf{20}   & \textbf{45}   & \textbf{80}   \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$         & $-4.68$       & $\bm{-4.97}$  & $\bm{-4.97}$  & $-4.83$       & $-4.11$       \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$         & $-3.12$       & $-3.46$       & $\bm{-3.55}$  & $-3.33$       & $-2.54$       \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$          & $-2.69$       & $\bm{-3.04}$  & $-2.77$       & $-2.25$       & $-1.91$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.88$       & $\bm{-5.16}$  & $-5.13$       & $-5.00$       & $-4.29$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.53$       & $\bm{-4.85}$  & $-4.79$       & $-4.60$       & $-3.95$       \\ \hline
%     $\text{VPT}_{dev}$ [s]/[steps]              & $0.52$/$6.50$ & $0.96$/$12.0$ & $0.98$/$12.3$ & $\bm{1.71}$/$21.4$ & $0.19$/$2.38$ \\ \hline
%     $\text{VPT}_{test,interp}$ [s]/[steps]      & $0.46$/$7.67$ & $\bm{0.87}$/$14.5$ & $0.78$/$13.0$ & $1.20$/$20.0$ & $0.17$/$2.83$ \\ \hline
%     $\text{VPT}_{test,extrap}$ [s]/[steps]      & $0.54$/$5.40$ & $1.07$/$10.7$ & $1.06$/$10.6$ & $\bm{1.58}$/$15.8$ & $0.19$/$1.90$
%     \end{tabular}
%     }
% \end{subtable}
% \end{table}

==> tables/batch_size_with_pinn_rollout_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!b]
\centering
\caption{Batch size experiment with physics and rollout loss.}
\label{tab:batch_size_with_pinn}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|r|r|r|}
\textbf{Batch Size}                         & \textbf{3}    & \textbf{10}   & \textbf{20}   & \textbf{45}   & \textbf{80}   \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $-4.68$       & $\bm{-4.97}$  & $\bm{-4.97}$  & $-4.83$       & $-4.11$       \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $-3.12$       & $-3.46$       & $\bm{-3.55}$  & $-3.33$       & $-2.54$       \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $-2.69$       & $\bm{-3.04}$  & $-2.77$       & $-2.25$       & $-1.91$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.88$       & $\bm{-5.16}$  & $-5.13$       & $-5.00$       & $-4.29$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.53$       & $\bm{-4.85}$  & $-4.79$       & $-4.60$       & $-3.95$       \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $0.52$/$6.50$ & $0.96$/$12.0$ & $0.98$/$12.3$ & $\bm{1.71}$/$21.4$ & $0.19$/$2.38$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $0.46$/$7.67$ & $\bm{0.87}$/$14.5$ & $0.78$/$13.0$ & $1.20$/$20.0$ & $0.17$/$2.83$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $0.54$/$5.40$ & $1.07$/$10.7$ & $1.06$/$10.6$ & $\bm{1.58}$/$15.8$ & $0.19$/$1.90$
\end{tabular}
}
\end{table}

==> tables/collocation_points_table.tex <==
% \begin{table}[!b]
% \centering
% \caption{Collocation points experiment}
% \label{tab:collocation_points}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|r|r|r|r}
% \textbf{Collocation Points} & \textbf{base} & \textbf{extra} & \textbf{extra b/a} & \textbf{no fixed} \\ \hline
% $\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.68}$  & $-4.17$       & $-3.95$       & $-4.57$       \\ \hline
% $\log_{10}(\mathcal{L}_{roll,dev})$         & $-3.12$       & $\bm{-3.27}$  & $-2.38$       & $-3.03$       \\ \hline
% $\log_{10}(\mathcal{L}_{phy,dev})$          & $-2.69$       & $\bm{-2.74}$  & $-1.86$       & $-2.25$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.88}$  & $-4.84$       & $-4.17$       & $-4.80$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.53$       & $\bm{-4.68}$  & $-3.78$       & $-4.37$       \\ \hline
% $\text{VPT}_{dev}$ [s]/[steps]              & $0.52$/$6.50$ & $\bm{1.45}$/$18.1$ & $0.30$/$3.75$ & $0.62$/$7.75$ \\ \hline
% $\text{VPT}_{test,interp}$ [s]              & $0.46$/$7.67$ & $\bm{0.86}$/$14.3$ & $0.28$/$4.67$ & $0.64$/$10.7$ \\ \hline
% $\text{VPT}_{test,extrap}$ [s]              & $0.54$/$5.40$ & $\bm{1.76}$/$17.6$ & $0.30$/$3.00$ & $0.61$/$6.10$
% \end{tabular}
% }
% \end{table}

==> tables/complex_data_table.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{graphicx}
% \begin{table}[!b]
% \centering
% \caption{Increased data complexity experiment}
% \label{tab:increased_data_complexity}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|r|r|r|r|r|r}
% \textbf{Physics Loss}                       & \textbf{no}    & \textbf{no}    & \textbf{yes}    & \textbf{yes}    & \textbf{yes}    & \textbf{yes}    \\ \hline
% \textbf{Rollout Loss}                       & \textbf{no}    & \textbf{no}    & \textbf{no}    & \textbf{no}    & \textbf{yes}    & \textbf{yes}    \\ \hline
% \textbf{Batch Size}                         & \textbf{3}    & \textbf{10}   & \textbf{3}    & \textbf{10}   & \textbf{3}    & \textbf{10}   \\ \hline
% \textbf{Complex dataset}         & \textbf{no}    & \textbf{yes}    & \textbf{no}    & \textbf{yes}    & \textbf{no}    & \textbf{yes}    \\ \hline
% $\log_{10}(\mathcal{L}_{data,dev})$         & $-3.04$       & $-4.42$       & $-3.04$       & $\bm{-4.62}$  & $-3.02$       & $-4.44$       \\ \hline
% $\log_{10}(\mathcal{L}_{roll,dev})$         & $-1.96$       & $-3.28$       & $-1.96$       & $\bm{-3.53}$  & $-1.95$       & $-3.39$       \\ \hline
% $\log_{10}(\mathcal{L}_{phy,dev})$          & $-0.56$       & $-0.97$       & $-0.58$       & $\bm{-2.35}$  & $-0.59$       & $-2.27$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-3.16$       & $-4.12$       & $-3.17$       & $\bm{-4.88}$  & $-3.14$       & $-4.56$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-2.93$       & $-3.96$       & $-2.93$       & $\bm{-4.41}$  & $-2.92$       & $-4.28$       \\ \hline
% $\text{VPT}_{dev}$ [s]/[steps]              & $0.08$/$1.00$ & $1.27$/$15.9$ & $0.12$/$1.50$ & $1.27$/$15.9$ & $0.05$/$0.63$ & $\bm{1.33}$/$16.6$ \\ \hline
% $\text{VPT}_{test,interp}$ [s]              & $0.04$/$0.67$ & $0.51$/$8.50$ & $0.14$/$2.33$ & $\bm{1.21}$/$20.2$ & $0.06$/$1.00$ & $1.22$/$20.3$ \\ \hline
% $\text{VPT}_{test,extrap}$ [s]              & $0.10$/$1.00$ & $0.50$/$5.00$ & $0.13$/$1.30$ & $\bm{1.33}$/$13.3$ & $0.06$/$0.60$ & $1.31$/$13.1$
% \end{tabular}
% }
% \end{table}

==> tables/gradient_method_table.tex <==
% \begin{table}[!b]
% \centering
% \caption{Gradient weighting experiment}
% \label{tab:grad_weighting}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|r|r|r}
% \textbf{Gradient Scaling Method} & \textbf{Normalization} & \textbf{ConFIG} & \textbf{Addition} \\ \hline
% $\log_{10}(\mathcal{L}_{data,dev})$         & $-4.85$       & $\bm{-5.12}$  & $-4.72$       \\ \hline
% $\log_{10}(\mathcal{L}_{roll,dev})$         & $-3.37$       & $\bm{-3.66}$  & $-3.17$       \\ \hline
% $\log_{10}(\mathcal{L}_{phy,dev})$          & $-2.67$       & $\bm{-2.90}$  & $-2.72$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.99$       & $\bm{-5.28}$  & $-4.76$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.70$       & $\bm{-4.94}$  & $-4.65$       \\ \hline
% $\text{VPT}_{dev}$ [s]/[steps]              & $1.51$/$18.9$ & $\bm{1.70}$/$21.3$ & $0.75$/$9.38$ \\ \hline
% $\text{VPT}_{test,interp}$ [s]/[steps]      & $1.27$/$21.2$ & $\bm{1.45}$/$24.2$ & $0.62$/$10.3$ \\ \hline
% $\text{VPT}_{test,extrap}$ [s]/[steps]      & $1.46$/$14.6$ & $\bm{1.73}$/$17.3$ & $0.89$/$8.90$
% \end{tabular}
% }
% \end{table}

==> tables/layer_norm_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!b]
\centering
\caption{Effect of layer normalization on performance metrics.}
\label{tab:layer_norm}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|}
\textbf{Layer Normalization}                & \textbf{With} & \textbf{Without} \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.68}$  & $-4.42$          \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $\bm{-3.12}$  & $-2.85$          \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-2.69}$  & $-2.36$          \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.88}$  & $-4.65$          \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $\bm{-4.53}$  & $-4.26$          \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $0.52$/$6.50$ & $\bm{0.81}$/$10.1$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $0.46$/$7.67$ & $\bm{0.82}$/$13.7$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $0.54$/$5.40$ & $\bm{0.79}$/$7.90$ 
\end{tabular}
%}
\end{table}

==> tables/losses_table.tex <==
% \begin{table}[!b]
% \centering
% \caption{Effect of physics, rollout, and IC losses on performance metrics}
% \label{tab:losses_included}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|r|r|r|r|r}
% \textbf{Physics/Rollout/IC} & \textbf{no/no/no} & \textbf{yes/no/no} & \textbf{no/yes/no} & \textbf{yes/yes/no} & \textbf{yes/yes/yes} \\ \hline
% $\log_{10}(\mathcal{L}_{data,dev})$         & $-4.45$       & $-4.85$       & $\bm{-5.02}$  & $-4.68$       & $-4.89$       \\ \hline
% $\log_{10}(\mathcal{L}_{roll,dev})$         & $-2.89$       & $-3.37$       & $\bm{-3.46}$  & $-3.12$       & $-3.40$       \\ \hline
% $\log_{10}(\mathcal{L}_{phy,dev})$          & $-1.84$       & $-2.67$       & $-1.82$       & $\bm{-2.69}$  & $-2.65$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.81$       & $-4.99$       & $-4.90$       & $-4.88$       & $\bm{-5.13}$  \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.16$       & $\bm{-4.70}$  & $-4.71$       & $-4.53$       & $-4.69$       \\ \hline
% $\text{VPT}_{dev}$ [s]/[steps]              & $0.46$/$5.75$ & $\bm{1.51}$/$18.9$ & $0.51$/$6.38$ & $0.52$/$6.50$ & $1.11$/$13.9$ \\ \hline
% $\text{VPT}_{test,interp}$ [s]/[steps]      & $0.42$/$7.00$ & $\bm{1.27}$/$21.2$ & $0.41$/$6.83$ & $0.46$/$7.67$ & $1.02$/$17.0$ \\ \hline
% $\text{VPT}_{test,extrap}$ [s]/[steps]      & $0.48$/$4.80$ & $\bm{1.46}$/$14.6$ & $1.36$/$13.6$ & $0.54$/$5.40$ & $1.18$/$11.8$
% \end{tabular}
% }
% \end{table}

==> tables/nn_size_table.tex <==
\begin{table}[!b]
\caption{Neural network size experiment.}
\label{tab:nn_size_exp}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|r|r|r|}
\textbf{NN Size $N_{layer}$/$N_h$}             & \textbf{4/32} & \textbf{3/32} & \textbf{5/32} & \textbf{4/16} & \textbf{4/64} \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$            & $-4.85$       & $-4.78$       & $-4.51$       & $\bm{-5.04}$  & $-4.93$       \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$            & $-3.37$       & $-3.27$       & $-2.94$       & $\bm{-3.56}$  & $-3.47$       \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$             & $-2.67$       & $-2.25$       & $-2.56$       & $\bm{-2.69}$  & $-2.60$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$    & $-4.99$       & $-4.90$       & $-4.69$       & $\bm{-5.24}$  & $-5.16$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$    & $-4.70$       & $-4.60$       & $-4.37$       & $\bm{-4.87}$  & $-4.74$       \\ \hline
$\text{VPT}_{dev}$ {[}s{]}/{[}steps{]}         & $\bm{1.51}$/$18.9$ & $1.23$/$15.4$ & $0.58$/$7.25$ & $1.36$/$17.0$ & $1.12$/$14$   \\ \hline
$\text{VPT}_{test,interp}$ {[}s{]}/{[}steps{]} & $1.27$/$21.2$ & $0.62$/$10.3$ & $0.46$/$7.67$ & $\bm{1.32}$/$22.0$ & $1.16$/$19.3$ \\ \hline
$\text{VPT}_{test,extrap}$ {[}s{]}/{[}steps{]} & $\bm{1.46}$/$14.6$ & $1.31$/$13.1$ & $0.58$/$5.8$  & $1.31$/$13.1$ & $1.11$/$11.1$
\end{tabular}%
}
\end{table}

==> tables/position_rotated_no_pinn_table.tex <==
\begin{table}[!b]
\centering
\caption{Structural physics information experiment, physics and rollout losses not included.}
\label{tab:position_rotated_no_pinn}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|}
\textbf{With physics informed architecture} & \textbf{yes}  & \textbf{no}   \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.45}$  & $-4.32$       \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $-2.89$       & $\bm{-3.37}$  \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-1.84}$  & $-2.67$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.81}$  & $-4.49$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $\bm{-4.16}$  & $-4.14$       \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $0.46$/$5.75$ & $\bm{0.50}$/$6.25$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $0.42$/$7.00$ & $\bm{0.49}$/$8.17$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{0.48}$/$4.80$ & $\bm{0.48}$/$4.80$
\end{tabular}
%}
\end{table}

==> tables/position_rotated_pinn_no_rollout_table.tex <==
\begin{table}[!hb]
\centering
\caption{Structural physics information experiment, physics loss included, rollout loss not included.}
\label{tab:position_rotated_pinn_no_rollout}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|}
\textbf{With physics informed architecture} & \textbf{yes}  & \textbf{no}   \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.85}$  & $-4.26$       \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $\bm{-3.37}$  & $-2.68$       \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-2.67}$  & $-2.17$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.99}$  & $-4.41$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $\bm{-4.70}$  & $-4.13$       \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $\bm{1.51}$/$18.9$ & $0.57$/$7.13$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $\bm{1.27}$/$21.2$ & $0.50$/$8.33$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{1.46}$/$14.6$ & $0.61$/$6.10$
\end{tabular}
%}
\end{table}

==> tables/position_rotated_pinn_rollout_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!b]
\centering
\caption{Structural physics information experiment, both physics and rollout losses included.}
\label{tab:position_rotated_pinn_rollout}
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|}
\textbf{With physics informed architecture} & \textbf{yes}  & \textbf{no}   \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.68}$  & $-4.17$       \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$         & $\bm{-3.12}$  & $-2.60$       \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-2.69}$  & $-2.00$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.88}$  & $-4.41$       \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$ & $\bm{-4.53}$  & $-3.99$       \\ \hline
$\text{VPT}_{dev}$ [s]/[steps]              & $0.52$/$6.50$ & $\bm{0.53}$/$6.63$ \\ \hline
$\text{VPT}_{test,interp}$ [s]/[steps]      & $0.46$/$7.67$ & $\bm{0.53}$/$8.83$ \\ \hline
$\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{0.54}$/$5.40$ & $0.50$/$5.00$
\end{tabular}
%}
\end{table}

==> tables/residual_connection_table.tex <==
\begin{table}[!b]
\caption{Residual Connection ablation experiment.}
\label{tab:ress_conn}
\centering
%\resizebox{\columnwidth}{!}{%
\begin{tabular}{l|r|r|}
\textbf{Residual Connection}                   & \textbf{With} & \textbf{Without} \\ \hline
$\log_{10}(\mathcal{L}_{data,dev})$            & $\bm{-4.85}$  & $-0.69$          \\ \hline
$\log_{10}(\mathcal{L}_{roll,dev})$            & $\bm{-3.37}$  & $2.09$           \\ \hline
$\log_{10}(\mathcal{L}_{phy,dev})$             & $\bm{-2.67}$  & $-0.83$          \\ \hline
$\log_{10}(\mathcal{L}_{data,test,interp})$    & $\bm{-4.99}$  & $-0.79$          \\ \hline
$\log_{10}(\mathcal{L}_{data,test,extrap})$    & $\bm{-4.70}$  & $-0.61$          \\ \hline
$\text{VPT}_{dev}$ {[}s{]}/{[}steps{]}         & $\bm{1.51}$/$18.9$ & $0.00$/$0.00$    \\ \hline
$\text{VPT}_{test,interp}$ {[}s{]}/{[}steps{]} & $\bm{1.27}$/$21.2$ & $0.00$/$0.00$    \\ \hline
$\text{VPT}_{test,extrap}$ {[}s{]}/{[}steps{]} & $\bm{1.46}$/$14.6$ & $0.00$/$0.00$   
\end{tabular}
%}
\end{table}



==> tables/scheduler_table.tex <==
% \begin{table}[b]
% \centering
% \caption{Adaptive learning rate scheduler experiment}
% \label{tab:scheduler}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{l|r|r|r|r|r|r}
% \textbf{Scheduler}                          & \textbf{no}   & \textbf{yes}  & \textbf{no}   & \textbf{yes}  & \textbf{no}   & \textbf{yes}  \\ \hline
% \textbf{Physics Loss}                       & \textbf{no}   & \textbf{no}   & \textbf{yes}  & \textbf{yes}  & \textbf{yes}  & \textbf{yes}  \\ \hline
% \textbf{Rollout Loss}                       & \textbf{no}   & \textbf{no}   & \textbf{no}   & \textbf{no}   & \textbf{yes}  & \textbf{yes}  \\ \hline
% $\log_{10}(\mathcal{L}_{data,dev})$         & $-4.45$       & $-5.21$       & $-4.85$       & $\bm{-5.62}$  & $-4.68$       & $-5.35$       \\ \hline
% $\log_{10}(\mathcal{L}_{roll,dev})$         & $-2.89$       & $-3.74$       & $-3.37$       & $\bm{-4.15}$  & $-3.12$       & $-3.92$       \\ \hline
% $\log_{10}(\mathcal{L}_{phy,dev})$          & $-1.84$       & $-1.78$       & $-2.67$       & $\bm{-3.30}$  & $-2.69$       & $-3.19$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,interp})$ & $-4.81$       & $-4.78$       & $-4.99$       & $\bm{-5.86}$  & $-4.88$       & $-5.44$       \\ \hline
% $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $-4.16$       & $-5.01$       & $-4.70$       & $\bm{-5.41}$  & $-4.53$       & $-5.30$       \\ \hline
% $\text{VPT}_{dev}$ [s]/[steps]              & $0.46$/$5.75$ & $1.43$/$17.9$ & $1.51$/$18.9$ & $2.53$/$31.6$ & $0.52$/$6.50$ & $\bm{2.76}$/$34.5$ \\ \hline
% $\text{VPT}_{test,interp}$ [s]              & $0.42$/$7.00$ & $0.51$/$8.50$ & $1.27$/$21.2$ & $\bm{2.56}$/$42.7$ & $0.46$/$7.67$ & $1.91$/$31.8$ \\ \hline
% $\text{VPT}_{test,extrap}$ [s]              & $0.48$/$4.80$ & $1.86$/$18.6$ & $1.46$/$14.6$ & $2.73$/$27.3$ & $0.54$/$5.40$ & $\bm{3.05}$/$30.5$
% \end{tabular}
% }
% \end{table}

==> tables/structure_subtables.tex <==
% \begin{table}[!b]
% \centering
% \caption{Structural physics-informed experiments}
% \label{tab:structure_experiments}
% \begin{subtable}{\columnwidth}
%     \centering
%     \caption{Without physics and rollout loss}
%     \label{tab:position_rotated_no_pinn}
%     %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r}
%     \textbf{With physics informed architecture} & \textbf{yes}  & \textbf{no}   \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.45}$  & $-4.32$       \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$         & $-2.89$       & $\bm{-3.37}$  \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-1.84}$  & $-2.67$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.81}$  & $-4.49$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $\bm{-4.16}$  & $-4.14$       \\ \hline
%     $\text{VPT}_{dev}$ [s]/[steps]              & $0.46$/$5.75$ & $\bm{0.50}$/$6.25$ \\ \hline
%     $\text{VPT}_{test,interp}$ [s]/[steps]      & $0.42$/$7.00$ & $\bm{0.49}$/$8.17$ \\ \hline
%     $\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{0.48}$/$4.80$ & $\bm{0.48}$/$4.80$
%     \end{tabular}
%         %}
% \end{subtable}

% \vspace{1em}

% \begin{subtable}{\columnwidth}
%     \centering
%     \caption{With physics loss, without rollout loss}
%     \label{tab:position_rotated_pinn_no_rollout}
%     %\resizebox{\columnwidth}{!}{%
%     \begin{tabular}{l|r|r}
%     \textbf{With physics informed architecture} & \textbf{yes}  & \textbf{no}   \\ \hline
%     $\log_{10}(\mathcal{L}_{data,dev})$         & $\bm{-4.85}$  & $-4.26$       \\ \hline
%     $\log_{10}(\mathcal{L}_{roll,dev})$         & $\bm{-3.37}$  & $-2.68$       \\ \hline
%     $\log_{10}(\mathcal{L}_{phy,dev})$          & $\bm{-2.67}$  & $-2.17$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,interp})$ & $\bm{-4.99}$  & $-4.41$       \\ \hline
%     $\log_{10}(\mathcal{L}_{data,test,extrap})$ & $\bm{-4.70}$  & $-4.13$       \\ \hline
%     $\text{VPT}_{dev}$ [s]/[steps]              & $\bm{1.51}$/$18.9$ & $0.57$/$7.13$ \\ \hline
%     $\text{VPT}_{test,interp}$ [s]/[steps]      & $\bm{1.27}$/$21.2$ & $0.50$/$8.33$ \\ \hline
%     $\text{VPT}_{test,extrap}$ [s]/[steps]      & $\bm{1.46}$/$14.6$ & $0.61$/$6.10$
%     \end{tabular}
% \end{subtable}
% \end{table}
